Dynamic Size Message Scheduling for Multi-Agent Communication under Limited Bandwidth

Communication plays a vital role in multi-agent systems, fostering collaboration and coordination. However, in real-world scenarios where communication is bandwidth-limited, existing multi-agent reinforcement learning (MARL) algorithms often provide agents with a binary choice: either transmitting a fixed number of bytes or no information at all. This limitation hinders the ability to effectively utilize the available bandwidth. To overcome this challenge, we present the Dynamic Size Message Scheduling (DSMS) method, which introduces a finer-grained approach to scheduling by considering the actual size of the information to be exchanged. Our contribution lies in adaptively adjusting message sizes using Fourier transform-based compression techniques, enabling agents to tailor their messages to match the allocated bandwidth while striking a balance between information loss and transmission efficiency. Receiving agents can reliably decompress the messages using the inverse Fourier transform. Experimental results demonstrate that DSMS significantly improves performance in multi-agent cooperative tasks by optimizing the utilization of bandwidth and effectively balancing information value.

==> introduction.tex <==

\emph{Multi-Agent Reinforcement Learning} (MARL) studies how the use of reinforcement learning (RL) to learn decentralized polices for multiple agent that interact in the same environment. These problems are common in real word applications where tasks involving sequential decision making cannot be solved by a unique agent. Examples of such problem include robot working in a warehouse, drones, and autonomous vehicles. While decentralization is usually required in multi-agent systems, it is common to include a limited communication medium in those systems to improve coordination and reduce partial observability. While some 
